EinDecomp: Decomposition of Declaratively-Specified Machine Learning and Numerical Computations for Parallel Execution

We consider the problem of automatically decomposing operations over tensors or arrays so that they can be executed in parallel on multiple devices. We address two, closely-linked questions. First, what programming abstraction should systems for tensor-based computing offer to enable such decompositions? Second, given that abstraction, how should such systems automatically decompose a tensor-based computation? We assert that tensor-based systems should offer a programming abstraction based on an extended Einstein summation notation, which is a fully declarative, mathematical specification for tensor computations. We show that any computation specified in the Einstein summation notation can be re-written into an equivalent tensor-relational computation, and this re-write generalizes existing notations of tensor parallelism such as "data parallel'' and "model parallel.'' We consider the algorithmic problem of optimally computing a tensor-relational decomposition of a graph of operations specified in our extended Einstein summation notation, and we experimentally show the value of the algorithm that we develop.

==> Assignments.tex <==




\subsection{Forming an \textsc{ExecGraph}}

How to form an \textsc{ExecGraph} from a \textsc{TaskGraph}? 
If the input \textsc{TaskGraph} consists of just a single EinSum computation, forming an \textsc{ExecGraph} is simple. As any binary EinSum computation is simply a join followed by an aggregation, the resulting \textsc{ExecGraph} will have two ``layers,'' the first showing the formation of tuples via the join, the second forming output tuples via an aggregation.  The various dataflow graphs in Figure 2 are effectively \textsc{ExecGraph}s.

How to link multiple EinSum computations together?  This is a question with a non-obvious answer, because of the (possible) need to re-partition tensors across EinSum computations.  Recall that Figure 4 shows one possible re-partition plan, though this particular plan has a large number of vertices, which may be problematic.
The tactic used by \texttt{Einsummable} is to combine both the aggregation in the first EinSum computation (if it exists) and the re-partition as part of the same subgraph.  To do this, we define the notion of a \emph{join group}.  Given the tuples $T^{(1)} = \{t^{(1)}_1, t^{(1)}_2, ....\}$ output from the join of the first EinSum operation, and the tuples $T^{(2)} = \{t^{(2)}_1, t^{(2)}_2, ....\}$ computed by the first EinSum operation that are input into the join of the second EinSum operation, we define the partitioning of $T^{(1)}$ and $T^{(2)}$ into \emph{join groups} via three rules:
\begin{enumerate}
\item Each tuple from $T^{(1)}$ and $T^{(2)}$ is in exactly one join group.
\item $t^{(1)}_i$ and $t^{(2)}_j$ are in the same join group if the tuple $t^{(1)}_i$ appears in the lineage of the computation of $t^{(2)}_j$.
\item $t^{(2)}_i$ and $t^{(2)}_j$ are not in the same group if there does not exist some $t^{(1)}_k$ that appears in the lineage of both $t^{(2)}_i$ and $t^{(2)}_j$.
\end{enumerate}
Consider the \textsc{ExecGraph} in Figure 6; there are two join groups connecting the two matrix multiples.

Figure 7 shows three graphs that implement the join groups of Figure 6.  In (a), the producer chunks are aggregated, and then the re-partition occurs, without the assumption that the final consumer chunks are constructed at a single location.  (c) is similar, but the assumption is that the construction of each consumer chunks take place at one location.  In (b), the aggregation \emph{and} the construction of each consumer chunk takes place at one location.  In \texttt{Einsummable} we choose option (b), as it is the simplest option, requiring choosing only the location of where the input join tuples are computed, as well as where the output tuples are computed.  We call the combined aggregation/formation of a consumer chunk a \emph{refinement} operation.




\subsection{An Optimization Problem for Placements}

Once an \textsc{ExecGraph} has been formed from a \textsc{TaskGraph}, the next step is to perform a \emph{placement}, where the vertices in the \textsc{ExecGraph} are placed onto machines so as to (a) ensure an even distribution of work, and (b) minimize communication between machines.  

For a vertex $v$ in the \textsc{ExecGraph}, let $v.\texttt{fp}$ denote the number of $\bigotimes$ calls in the operation. For the purpose of defining the placement problem, the set of edges (representing data flow) is represented as a map $E$ from (vertex, vertex) pairs to the  set $\{0, 1\}$. A 0 indicates that there is not a flow from the first vertex to the second, while a 1 indicates that there is.  Let a \emph{placement} $\mathcal{P}$ be a map from all (vertex, location) pairs to the set $\{0, 1\}$; a 0 indicates that the vertex was not placed at the given location, and a 1 indicates that it was. Then, optimizing the placement requires solving the following mini-max optimization problem: $\substack{\textrm{argmin} \\ \mathcal{P}} \hspace{5 pt} Cost(\mathcal{P})$ where $Cost(\mathcal{P})$ is:
\begin{align}\substack{\textrm{max} \\ l} \bigg( \sum_v \mathcal{P}[l, v] \times  \Big(  \alpha \times v.\texttt{fp } + 
\sum_{v'} E[v, v'] \times (1 - \mathcal{P}[l, v']) \times v.\texttt{sz } + \nonumber \\
\sum_{v'} E[v', v] \times (1 - \mathcal{P}[l, v']) \times v'.\texttt{sz}   \Big) \bigg)  \nonumber \end{align}
\noindent We minimize expensive site cost.  The cost for a site is the number of floating point operations run on the machine, plus the number of bytes transferred into and out of the site.  A multiplier $\alpha$ discounts the floating point operation cost, compared to the transfer cost.



\subsection{Solving the Placement Problem}

The unique structure of the \textsc{ExecGraph}---it is a DAG of exploded EinSum operations---seems to make it amenable to a greedy assignment algorithm proceeds from EinSum operation to EinSum operation through the \textsc{ExecGraph}, assigning vertices.  This is exactly what we do in \texttt{Einsummable}.  We start with the input tensor relations, and assign all of the input tuples in reach tensor relation to machines, round-robin, taking care to choose the same lexicographic ordering of tuples---enumerating them along the first dimension, then the second, then the third, and so on.  This produces a partial assignment, which we store in $\mathcal{P}$.

Then, we choose one EinSum operation where both of its inputs have been placed (or, in the case of a unary EinSum operation, where its input has been placed).  Let $V^{(1)}$ be the set of \textsc{ExecGraph} vertices  computing the tuples resulting from the join within the EinSum operation, and let Let $V^{(2)}$ be the set of refinement operations that operate over tuples produced by $V^{(1)}$.  We call \textsc{HandleNewEinSum}$(\mathcal{P}$, $L$, $V^{(1)}$, $V^{(2)})$ to produce a new version of $\mathcal{P}$ that includes a placement for both $V^{(1)}$ and $V^{(2)}$.  Here, $L$ is the number of locations, or machines.  Pseudo-code for \textsc{HandleNewEinSum} is given in Algorithm 1. This is done repeatedly, until all of the EinSum operations have been placed.

\textsc{HandleNewEinSum} works by first partitioning  $V^{(1)}$ and $V^{(2)}$ into join groups\footnote{Note that while the notion of a join group was defined over tuples, we abuse this notion slightly and assume that it naturally extends to the \textsc{ExecGraph} vertices that compute those tuples.}  Then, for each join group, the algorithm enumerates possible placements, and greedily chooses the best.  
It is not feasible to enumerate all of them, as there are combinatorially many: $L$ machines and $p$ tuples in the join group, there are our $p^L$.  Our implementation considers at most $2L - 1$ placements.  We do this by partitioning the $L$ machines into $1$ groups of $L$ machines and doing a round-robin placement, then by partitioning into $2$ groups of $L/2$ machines and considering a round-robin placement within each possible group, then by partitioning into $4$ groups of $L/4$ machines and considering a round-robin placement within each possible group, and so on.  So if we had $8$ tuples to compute in a join and $L = 4$, the possible assignment vectors for those $8$ tuples would be:
$\langle 00000000 \rangle$, 
$\langle 11111111 \rangle$, 
$\langle 22222222  \rangle$, 
$\langle 33333333  \rangle$, 
$\langle 01010101  \rangle$, 
$\langle 23232323  \rangle$, 
$\langle 01230123 \rangle$.  The algorithm to enumerate the possible placements is given as \textsc{Enumerate} in Algorithm 1.







==> Einstein.tex <==



In frameworks such as TensorFlow and PyTorch, programmers link together  operations over tensors. However, there is little separation between the programming abstraction and the implementation abstraction---a programmer specifies a set of black-box operations to run, and (more or less) those are the operations that are actually executed.  Hence, the underlying system cannot reason about the computation.  Further, there are a lot of operations available to an ML programmer, so it makes implementing this programming abstraction difficult.  As the PyTorch documentation says, ``Writing a backend for PyTorch is challenging. PyTorch has 1200+ operators, and 2000+ if you consider various overloads for each operator \cite{backend}.''

If the goal is to separate the programming abstraction from the implementation abstraction---as has classically been done in relational systems, the question becomes: what should these abstractions be in ML systems?  

\subsection{Programming Abstraction}

While SQL is synonymous with relational programming, it is unlikely to be adopted as a standard language for ML programming---even if tensors are in fact relations. It is ``wordy'' (inherited from COBOL) and not natural for mathematical programming.

A reasonable programming abstraction for relational systems is an extended variant of Einstein summation notation (or ``EinSum'') \cite{blacher2023efficient,laue2020simple,einstein1938gravitational}, which is already supported to at least a rudimentary extent by PyTorch \cite{rogozhnikov2021einops}. Using EinSum, it is quite natural to specify a wide variety of ML computations, including modern transformers.  And crucially, EinSum makes it possible for the underlying system to ``understand'' the underlying computation. 

We begin our discussion of the EinSum language by defining the notion of a \emph{tensor}.  We use bold upper-case (for example, $\textbf{U}$) to denote a tensor.
Define the \emph{bound} vector for $\textbf{U}$, $\textbf{b}_\textbf{U}$, to be a vector of integers of length $r$.  ``$r$'' stands for ``rank.'' Next, define $\mathcal{I}(\textbf{b}_\textbf{U})$ to be the set $\{0...\textbf{b}_\textbf{U}[0] - 1\} \times \{0...\textbf{b}_\textbf{U}[1] - 1\} \times ..., \times \{0...\textbf{b}_\textbf{U}[r-1] - 1\}$.  This is the set of all indices or keys that obey the bound.  For example, if $\textbf{b}_\textbf{U} = \langle 2, 3, 4 \rangle$ then $\langle 1, 2, 3 \rangle$ is in  $\mathcal{I}(\textbf{b}_\textbf{U})$, because $1 \in \{0, 1\}$, $2 \in \{0, 1, 2\}$, and $3 \in \{0, 1, 2, 3\}$.  When we need to concatenate the bound vectors for tensors $\textbf{X}$ and $\textbf{Y}$, we use the notation $\textbf{b}_{\textbf{X} \textbf{Y}}$.
A tensor $\textbf{U}$ is then a function from $\mathcal{I}(\textbf{b}_\textbf{U})$ 
to the set of real numbers.

We next introduce the notion of a \emph{label}, which is just some symbol that can be bound to a value.  We use $\ell_\textbf{U}$ to denote a list (vector) of labels used to index into tensor $\textbf{U}$.  Viewed relationally, a tensor with label vector $\ell_\textbf{U}$ is equivalent to a database relation with schema $\textbf{U}(\ell_\textbf{U}[1], \ell_\textbf{U}[2], ..., \texttt{val})$. When we ``bind'' $\ell_\textbf{U}$, we are specifying specific key values we are interested in selecting for. 
To denote the concatenation of two label lists $\ell_\textbf{X}$ and $\ell_\textbf{Y}$, we use $\ell_\textbf{XY}$.

Given this, the following EinSum sums up all of the entries in $\textbf{U}$:
$$\textbf{V}_\emptyset \leftarrow \sum_{\ell_\textbf{U} \in \mathcal{I}(\textbf{b}_\textbf{U})}  \textbf{U}_{\ell_{\textbf{U}}}$$ 
$\textbf{V}_\emptyset$ means that tensor $\textbf{V}$ does not need an index, so it is a scalar. 

However, Einsum can describe much more complicated computations.  Often, we will need to project/permute a bound vector.  
Given two lists of labels $\ell_1$ and $\ell_2$, and a bound vector $\textbf{b}$, define $\textbf{b}[\ell_1; \ell_2]$ 
to be a vector of length $|\ell_1|$, where the $i$th entry is $\textbf{b}[j]$ iff $\ell_1[i]$ = $\ell_2[j]$.  
As an example, let us again assume $\textbf{b} = \langle 2, 3, 4 \rangle$ and let $\ell_1 = \langle k, i \rangle$ and $\ell_2 = \langle i, j, k \rangle$.  Then $\textbf{b}[\ell_1; \ell_2] = \langle 4, 2 \rangle$. 

Given this, binary Einsum expressions take the general form:
\begin{align}
\forall \hspace{2 pt} \ell_\textbf{Z} \in 
\mathcal{I}\left(\textbf{b}_{\textbf{Z}} \right): 
\hspace{2 pt} \textbf{Z}_{\ell_\textbf{Z}} \leftarrow
\bigoplus_{\ell_\textrm{agg} \in \mathcal{I} \left( \textbf{b}_{\textbf{X} \textbf{Y}}[\ell_{\textrm{agg}}; \ell_{\textbf{X} \textbf{Y}}] \right)} & \left( \bigotimes \left( \textbf{X}_{\ell_\textbf{X}}, \textbf{Y}_{\ell_\textbf{Y}} \right) \right) \end{align}
\noindent Here, $\bigoplus$ is a commutative/associative operation (most often addition) and $\bigotimes$ is some function (most often multiplication). If $\ell_\textrm{agg}$ is not empty (meaning one or more indices are being summed out), then the EinSum is often referred to as a \emph{contraction}.  If $\ell_\textbf{Z}$ contains labels not found in $\ell_\textbf{X}$ and/or $\ell_\textbf{Y}$, then the EinSum is often referred to as a \emph{broadcast}, as entries are being replicated across one or more dimensions.  In the remainder of the paper, we ignore broadcasts (so $\textbf{b}_\textbf{Z} = \textbf{b}_{\textbf{XY}}[\ell_\textbf{Z}; \ell_\textbf{XY}]$) and focus on contractions, as they tend to be computationally challenging.  We assume no repeated labels in $\ell_\textbf{X}$ or in $\ell_\textbf{Y}$, but labels are often repeated across the two sets.

For a concrete example of this, consider matrix multiplication of \textbf{X} and \textbf{Y}, with $\textbf{b}_\textbf{X} = [10, 50]$ and $\textbf{b}_\textbf{Y} = [50, 100]$:
\begin{align}
\forall \hspace{2 pt} i,k \in 
\mathcal{I}\left([10, 100])\right): & 
\hspace{5 pt} \textbf{Z}_{i,k} \leftarrow 
\sum_{j \in \mathcal{I} \left( [50] \right)}  \textbf{X}_{i,j} \times \textbf{Y}_{j,k} \nonumber \end{align}
EinSum can be simplified if we do not state the bounds and do not label the summation with $\ell_\textrm{agg}$, whose value is implicit: any indices in $\ell_\textbf{X}$ or $\ell_\textbf{Y}$ that do not appear in $\ell_\textbf{Z}$ must appear in $\ell_\textrm{agg}$.  

We can construct EinSum expressions out of any number of input tensors and string them together to build complicated computations, though unary and binary EinSum expressions are most common, and are the expressions we consider in this paper.  Here are a sequence of EinSum expressions that implement a feed forward neural network with a single hidden layer:
\begin{align}
    &\textbf{A}_{i} \leftarrow \sum  \textbf{X}_{i,j} \times  \textbf{W}_{i,j}^{(1)}  \hspace{.2 cm}
    \textbf{B}_{i,j} \leftarrow \textrm{ReLU} ( \textbf{A}_{i,j}) \hspace{.2 cm}
    \textbf{C}_{i} \leftarrow \sum \textbf{B}_{i,j} \times  \textbf{W}_{j,k}^{(2)} \nonumber \\
    &\textbf{D}_i \leftarrow \sum \exp (\textbf{C}_{i,j}) \hspace{.2 cm}
    \textbf{E}_{i,j} \leftarrow \frac{\exp(\textbf{C}_{i,j})} {\textbf{D}_{i}} \nonumber 
\end{align}
\noindent For clarity, in the above expression, when no attributes are being summed over, we drop the summation.

This computation can be represented as a directed, acyclic graph called an \textsc{EinGraph} whose nodes are EinSum expressions and whose edges represent data flow.  For each vertex, we have a triple: 
$$(\texttt{bound}, \texttt{EinSum}, \texttt{inputs})$$
\texttt{EinSum} is the code run at the vertex, \texttt{bound} is the bound vector $\textbf{b}$ for the output of the \texttt{EinSum}, and \texttt{inputs} lists vertices providing inputs to this vertex.  Note that \texttt{inputs} has an explicit ordering, as EinSum need not be commutative.  \texttt{inputs} is empty if and only if \texttt{EinSum} is an empty string; then the tensor is input to the computation.

\subsection{Implementation Abstraction}

EinSum is just a relational programming language, like SQL.  Thus, one might assume that the correct implementation abstraction for EinSum is relational algebra (RA), which has served this role in relational databases for more than 40 years.  There is no conceptual problem with this. A binary EinSum expression over tensors $\textbf{X}$ and $\textbf{Y}$ specifies a natural join of $\textbf{X}$ and $\textbf{Y}$ with an (optional) aggregation.

However, classical RA is not a reasonable implementation abstraction for ML as a system based purely on classical RA will be far too slow.  Unless a system can make use of  optimized codes for operations such as matrix multiplication which are highly-tuned for a specific processor and sometimes orders of magnitude faster than a naive implementation, it is unlikely to be competitive.

For this reason, we advocate for a ``tensor relational algebra''  (TRA) \cite{YuanJZTBJ21} as the proper implementation abstraction.  At the highest level, rather than storing a tensor $\textbf{U}$ as a set of $\prod_i \textbf{b}_\textbf{U}[i]$ tuples, given a partitioning vector $\textbf{d}$, we store a tensor ``tensor-relationally''. That is, we slice the $i$th dimension $\textbf{d}[i]$ ways, creating $\prod_i \textbf{d}[i] \leq \prod_i \textbf{b}_\textbf{U}[i]$ ``chunks'', and store each of those chunks in a tuple, with a key that identifies the chunk. The benefit of this approach is that high-performance operations or ``kernels'', such as highly-tuned matrix multiplications specialized to the hardware can be used over the chunks stored in the resulting relation.

To examine how arbitrary EinSum expressions can be implemented as tensor-relational computations, let us formalize the idea of partitioning or slicing up a tensor according to the vector $\textbf{d}$, and operating over such a tensor using EinSum. 

Rather than having one list of labels $\ell_\textbf{U}$ that visits all entries in a tensor by binding to the values in $\mathcal{I} (\textbf{b}_\textbf{U})$, we instead have two lists of labels $\ell_\textbf{U}$ and $\bar{\ell}_\textbf{U}$.  The ``bar'' operation adds an extra annotation to each label in $\ell_\textbf{U}$, creating a new label such that two labels are equivalent after the ``bar'' operation if and only if they were equivalent before the ``bar'' operation.  $\ell_\textbf{U}$ binds to the values in $\mathcal{I} (\textbf{d})$, and $\bar{\ell}_\textbf{U}$ binds to the values in $\mathcal{I} (\textbf{b}_\textbf{U} / \textbf{d})$ (we assume that arithmetic operations such as $/$ over vectors operate item-wise). So, to sum up all of the entries in a tensor, we would write:
$$
\textbf{V}_\emptyset \leftarrow \sum_{\substack{\ell_\textbf{U} \in \mathcal{I}(\textbf{d}) \\  \bar{\ell}_\textbf{U} \in \mathcal{I}(\textbf{d} / \textbf{b}_\textbf{U})}} \textbf{U}_{\ell_{\textbf{U}} \times \textbf{d} +  \bar{\ell}_\textbf{U}}
$$
Now, consider partitioning a binary EinSum computation using a partition vector $\textbf{d}$.  We can now re-write a binary EinSum expression of the form given in (1) as:
\begin{align}
&\forall \ell_\textbf{Z} \in 
\mathcal{I}\left(\textbf{d}\left[\ell_{\textbf{Z}}; \ell_{\textbf{X} \textbf{Y}}\right]\right), \bar{\ell}_\textbf{Z} \in 
\mathcal{I} \left( \frac{\textbf{b}_{\textbf{X} \textbf{Y}}} {\textbf{d}} \left[ \ell_{\textbf{Z}}; \ell_{\textbf{X} \textbf{Y}} \right] \right): 
 \textbf{Z}_{\ell_\textbf{Z} \times \frac{\textbf{b}_{\textbf{X} \textbf{Y}}} {\textbf{d}}\left[\ell_{\textbf{Z}}; \ell_{\textbf{X} \textbf{Y}} \right] + \bar{\ell}_\textbf{Z} } \nonumber 
\\
&\leftarrow  \bigoplus_{\substack{\ell_\textrm{agg} \in \mathcal{I} \left( \textbf{d} [ \ell_{\textrm{agg}} ; \ell_{\textbf{X} \textbf{Y}}] \right) \\ \bar{\ell}_\textrm{agg} \in \mathcal{I} \left( \frac{\textbf{b}_{\textbf{X} \textbf{Y}}} {\textbf{d}} [ \ell_{\textrm{agg}} ; \ell_{\textbf{X} \textbf{Y}}] \right)}}
\hspace{-10 pt} \bigotimes \left( \textbf{X}_{\ell_\textbf{X} \times \textbf{d} [\ell_\textbf{X}, \ell_\textbf{XY}] + \bar{\ell}_\textbf{X}},
\textbf{Y}_{\ell_\textbf{Y} \times \textbf{d} [\ell_\textbf{Y}; \ell_\textbf{XY}] + \bar{\ell}_\textbf{Y}} \right) 
\end{align}
Now, assume that $\mathcal{Z}$, $\mathcal{X}$, and $\mathcal{Y}$ are \emph{tensor relational} representations of $\mathbf{Z}$, $\mathbf{X}$, and $\mathbf{Y}$ where $\mathcal{Z}^{\ell_\textbf{Z}}_{\bar{\ell}_\textbf{Z}} = \textbf{Z}_{\ell_\textbf{Z} \times \frac{\textbf{b}_{\textbf{X} \textbf{Y}}} {\textbf{d}}\left[\ell_{\textbf{Z}}; \ell_{\textbf{X} \textbf{Y}} \right] + \bar{\ell}_\textbf{Z} }$. $\mathcal{X}$, and $\mathcal{Y}$ are defined similarly.  That is, the input tensor is partitioned according to $\textbf{d}$ we use the key $\ell_\textbf{Z}$ to select a particular chunk from a tensor relation, and then $\bar{\ell}_\textbf{Z}$ is used to index into that relation.  Now, we can re-write (2) as:
\begin{align}
\forall \ell_\textbf{Z} \in 
\mathcal{I}\left(\textbf{d}\left[\ell_{\textbf{Z}}; \ell_{\textbf{X} \textbf{Y}}\right]\right), \bar{\ell}_\textbf{Z} \in 
\mathcal{I} \left( \frac{\textbf{b}_{\textbf{X} \textbf{Y}}} {\textbf{d}} \left[ \ell_{\textbf{Z}}; \ell_{\textbf{X} \textbf{Y}} \right] \right): 
\mathcal{Z}^{\ell_\textbf{Z}}_{\bar{\ell}_\textbf{Z}} \nonumber 
\\
\leftarrow  \bigoplus_{\substack{\ell_\textrm{agg} \in \mathcal{I} \left( \textbf{d} [ \ell_{\textrm{agg}} ; \ell_{\textbf{X} \textbf{Y}}] \right) \\ \bar{\ell}_\textrm{agg} \in \mathcal{I} \left( \frac{\textbf{b}_{\textbf{X} \textbf{Y}}} {\textbf{d}} [ \ell_{\textrm{agg}} ; \ell_{\textbf{X} \textbf{Y}}] \right)}}
\bigotimes \left( \mathcal{X}^{\ell_\textbf{X}}_{\bar{\ell}_\textbf{X}},
\mathcal{Y}^{\ell_\textbf{Y}}_{\bar{\ell}_\textbf{Y}} \right) \nonumber
\end{align}
Note that we effectively have a nested EinSum expression: the outer one is operating over tensor relations, and the inner one is operating over tensors in those two tensor relations. 

\begin{figure}[t]
\includegraphics[width=8.5cm]{Partitionings.png}
\vspace{-15 pt}
 \caption{Four tensor-relational partitionings for  $\textbf{Z}_{i,k} \leftarrow \sum \textbf{X}_{i,j} \times \textbf{Y}_{j,k}$. In each there are 16 kernel calls. }
 \vspace{-5 pt}
 \label{fig:schsys}
\end{figure}


\begin{figure*}[th!]
\includegraphics[width=18cm]{Compute_Plans.png}
\vspace{-18 pt}
 \caption{Dataflow graphs associated with the partitionings of Figure 1. For partitionings $\textbf{d} = [4, 1, 1, 4]$ and  $\textbf{d} = [2, 1, 1, 8]$, there is only a join layer, as the joined dimensions are not partitioned.  For $\textbf{d} = [2, 4, 4, 2]$ and  $\textbf{d} = [2, 2, 2, 4]$ there is also an aggregation. }
 \vspace{-5 pt}
 \label{fig:schsys}
\end{figure*}

Now, imagine that we have a \emph{kernel function} $K$ that accepts two sub-tensors from $\mathcal{X}$ and $\mathcal{Y}$ and computes the inner EinSum expression over them. That is, $K()$ accepts two input chunks $\mathcal{X}^{\ell_\textbf{X}}$ and $\mathcal{Y}^{\ell_\textbf{Y}}$ and creates a tensor $\textbf{Z}'$ with bound vector $\frac{\textbf{b}_{\textbf{X} \textbf{Y}}} {\textbf{d}}$  such that $\forall \bar{\ell}_\textbf{Z} \in 
\mathcal{I} \left( \frac{\textbf{b}_{\textbf{X} \textbf{Y}}} {\textbf{d}} \left[ \ell_{\textbf{Z}}; \ell_{\textbf{X} \textbf{Y}} \right] \right)$,
$\textbf{Z}'_{\bar{\ell}_\textbf{Z}}$ 
is set to 
$\bigoplus_{ \bar{\ell}_\textrm{agg} \in \mathcal{I} \left( \frac{\textbf{b}_{\textbf{X} \textbf{Y}}} {\textbf{d}} [ \ell_{\textrm{agg}} ; \ell_{\textbf{X} \textbf{Y}}] \right)}
\bigotimes \left( \mathcal{X}^{\ell_\textbf{X}}_{\bar{\ell}_\textbf{X}},
\mathcal{Y}^{\ell_\textbf{Y}}_{\bar{\ell}_\textbf{Y}} \right)$   If $\bigoplus$ over two tensors performs the $\bigoplus$ operation element-wise over entries in the tensors, then, using this kernel, (2) becomes:
\begin{align}
\forall \ell_\textbf{Z} \in 
\mathcal{I}\left(\textbf{d}\left[\ell_{\textbf{Z}}; \ell_{\textbf{X} \textbf{Y}}\right]\right): 
\mathcal{Z}^{\ell_\textbf{Z}} \leftarrow \hspace{-10 pt} \bigoplus_{\ell_\textrm{agg} \in \mathcal{I} \left( \textbf{d} [ \ell_{\textrm{agg}} ; \ell_{\textbf{X} \textbf{Y}}] \right)}
K \left( \mathcal{X}^{\ell_\textbf{X}},
\mathcal{Y}^{\ell_\textbf{Y}} \right)
\end{align}
Thus, we have shown that any binary EinSum expression can easily be re-written as an equivalent, tensor-relational computation. For example, a tensor-relational implementation of matrix multiplication of two $100 \times 100$ matrices, decomposed into $20 \times 20$ chunks via partitioning vector $\textbf{d} = [5, 5, 5, 5]$ is 
$\forall i, k \in 
\mathcal{I}\left( [5, 5] \right): 
\mathcal{Z}^{i, k} \leftarrow  \sum_{j \in \mathcal{I} \left( [5] \right)}
K \left( \mathcal{X}^{i,j},
\mathcal{Y}^{j,k} \right)$.  Note that (3) is still implemented as a natural join followed by an aggregation, though now it is a natural join and an aggregation of tensor relations.



\vspace{5 pt}
\noindent
\textbf{A note on kernel functions.}   \texttt{Einsummable} requires the ability to generate a high-performance, hardware-specific kernel function implementations of each EinSum. We found the best option was to develop our own kernel compiler, which uses a cost model to choose the best unrolling of the EinSum expression, executing it as a sequence of calls to an Intel MKL \cite{wang2014intel} matrix multiply. 

==> Engine.tex <==

\begin{figure}[t]
\includegraphics[width=8.5cm]{ExecGraph.png}
\vspace{-20 pt}
 \caption{Creating an \textsc{ExecGraph}.  This example considers a sequence of two matrix multiplications.   }
 \vspace{-5 pt}
 \label{fig:schsys}
\end{figure}


\begin{figure}[t]
\includegraphics[width=8.5cm]{RepartitionOptions.png}
\vspace{-15 pt}
 \caption{Different compilation options for the aggregation/repartition.  (b) is the option chosen in the current \texttt{Einsummable} implementation.   }
 \vspace{-5 pt}
 \label{fig:schsys}
\end{figure}

\subsection{Why Not a Classical Database Engine?}

Once an EinSum expression has been transformed into a tensor-relational calculation, it must be executed. We argue that a classical database engine is the wrong choice.  Such engines assume that determining how tuples contribute to the operator's output is potentially costly and must be optimized---for example, relational systems assume the difficulty in processing a binary join is in determining which tuples from the left input relation match which tuples from the right. This assumption does not hold in an EinSum computation, where the input tuples can be massive and it is not difficult to know how they link. The result is poor performance.

Re-consider the example matrix multiply SQL query from the introduction, which uses the \texttt{matrix\_multiply} kernel.
Consider running this on a classical relational system, with 64 processors.  Assume the input matrices (both $8000 \times 8000$) have been chunked 16 ways (into 16, $2000 \times 2000$ chunks).  
To execute this query using a classical hash join, we would hash all input tuples on \texttt{B.colID} \texttt{=} \texttt{C.rowID}. However, we immediately run into a problem, as there are only four \texttt{B.colID}/\texttt{C.rowID} values.  We cannot utilize 64 processors.

In contrast, note that if we were to manually assign each of the 64 pairwise \texttt{matrix\_multiply} kernel calls to one of the 64 processors, then each processor would run exactly one of the \texttt{matrix\_multiply} kernels. Costing the join and aggregation using the formulas of Section 4 gives us 704 million floating point numbers transferred.

Even if we require that all 64 processors be utilized, a database engine cannot perform as well. For example, a hash join can keep all processors busy if we slice $\textbf{B}$ 64 ways vertically, and 4 ways horizontally, (while $\textbf{C}$ is sliced 4 ways vertically, and 64 ways horizontally).  In this way, each one of 64 \texttt{B.colID} \texttt{=} \texttt{C.rowID} values can be mapped to a different processor by a standard hash join, and all processors are busy during the join.  However, using the formulas from section 4, this gives us an upper bound of 4.16 billion numbers transferred, or more than seven times the cost of the prior solution.


\begin{algorithm}[t]
\begin{algorithmic}[1]
\Function{HandleNewEinSum}{$\mathcal{P}$, $L$, $V^{(1)}$, $V^{(2)}$}
\State \textbf{partition} $V^{(1)}$ and $V^{(2)}$ into join groups $(G^{(1)}_1, G^{(2)}_1)$,\\
\hspace{13 pt} $(G^{(1)}_2, G^{(2)}_2), ...$, where each $(G^{(1)}_i, G^{(2)}_i)$ are the subsets \\
\hspace{13 pt} of $V^{(1)}$ and $V^{(2)}$ appearing in the $i$th join group
\State \textbf{for} each $i$
\State \hspace{10 pt} $\mathcal{P} \leftarrow \textsc{DoAssign} (\mathcal{P}, L, G^{(1)}_i, G^{(2)}_i)$
\State \textbf{return} $\mathcal{P}$
\EndFunction

\vspace{5 pt}
\Function{DoAssign}{$\mathcal{P}$, $L$, $G^{(1)}$, $G^{(2)}$}
\State $best \leftarrow \infty$; $all \leftarrow  \textsc{Enumerate} (p, G^{(1)})$
\State \textbf{for} $a \in all$ do:
\State \hspace{10 pt} \textbf{for} $i \in \{0, ..., |G^{(1)}|\}$ do: 
\State \hspace{20 pt} $\mathcal{P}[a[i], G^{(1)}[j]] \leftarrow 1$ if $j = i$; $\leftarrow 0$ otherwise 
\State \hspace{20 pt} \textbf{for} $i \in \{0, ..., |G^{(2)}|\}$ do:
\State \hspace{30 pt} \textbf{choose} location $l$ to set $\mathcal{P}(l, G^{(2)}[i]) \leftarrow 1$, \\
\hspace{43 pt} $\mathcal{P}(l' \neq l, G^{(2)}[i] \leftarrow 0$ so as to minimize $Cost(\mathcal{P})$
\State \hspace{20 pt} \textbf{if} $Cost(\mathcal{P})$ < $best$ \textbf{then} $\mathcal{P}^* \leftarrow \mathcal{P}$; $best \leftarrow Cost(\mathcal{P})$
\State \textbf{return} $\mathcal{P}^*$
\EndFunction

\vspace{5 pt}
\Function{Enumerate}{$L$, $numJoins$}
\State  $list \leftarrow []$
\State \textbf{for} $width \in \{1, 2, 4, 8, ..., >\}$
\State \hspace{10 pt}  \textbf{if} $width > numJoins$ \textbf{then} break;
\State \hspace{10 pt} \textbf{while} $i < L$
     \State \hspace{20 pt} $cur \leftarrow i;  limit \leftarrow i + width$
     \State \hspace{20 pt} \textbf{for} $j \in \{0, ..., numJoins - 1\}$
        \State \hspace{30 pt} $t[j] \leftarrow cur$;
        $cur++$
        \State \hspace{30 pt} \textbf{if} $cur = limit$ \textbf{then} $cur \leftarrow i$
         \State \hspace{20 pt} \textbf{append} $t$ to $list$; $i \leftarrow i + width$
\State \textbf{return} $list$
 \EndFunction
\end{algorithmic}
\caption{Algorithm for performing a placement of the computation of join tuples for one additional EinSum operation. }
\end{algorithm}



\begin{figure*}[t]
    \centering
    \begin{minipage}{.25\textwidth}
        \centering
        \setlength\tabcolsep{3pt}
\begin{tabular}{|cccc|}
\multicolumn{4}{c}{Batch size 1, 7B params} \\
\hline
Num \vspace{-2 pt} & Time & FLOPS & FLOPS \vspace{-2 pt} \\ 
 Mach. &  &  & /mach. \\ 
       \hline
1 &	4.04 & 8.38e12 &  8.38e11 \\
2 &	2.76 & 1.22e12 & 6.13e11 \\
4 &	2.98 & 1.13e12 &  2.84e11 \\
8 & 2.28 & 1.49e12 & 1.86e11 \\
       \hline
\end{tabular}

\end{minipage}%
    \begin{minipage}{.25\textwidth}
    \centering \setlength\tabcolsep{3pt}
\begin{tabular}{|cccc|}
\multicolumn{4}{c}{Batch size 4, 7B params} \\
\hline
Num \vspace{-2 pt} & Time & FLOPS & FLOPS \vspace{-2 pt} \\ 
 Mach. & (secs) &  & /mach. \\ 
       \hline
1 &	11.4 & 1.19e12 &  1.19e12 \\
2 &	7.30 & 1.86e12 & 9.28e11 \\
4 &	5.07 & 2.67e12 & 6.68e11 \\
8 &	3.79 & 3.57e12 &  4.47e11 \\
       \hline
\end{tabular}

    \end{minipage}%
    \begin{minipage}{.25\textwidth}
        \centering   \setlength\tabcolsep{3pt}
\begin{tabular}{|cccc|}
\multicolumn{4}{c}{Batch size 16, 7B params} \\
\hline
Num \vspace{-2 pt} & Time & FLOPS & FLOPS \vspace{-2 pt} \\ 
 Mach. & (secs) &  & /mach. \\ 
       \hline
1 &	42.0 & 1.29e12 &  1.29e12 \\
2 &	24.4 & 2.22e12 & 1.11e12 \\
4 &	15.21 & 3.56e12 &  8.90e11 \\
8 &	8.88 & 6.10e12 &  7.62e11 \\
       \hline
\end{tabular}
    \end{minipage}%
    \begin{minipage}{.25\textwidth}
        \centering \setlength\tabcolsep{3pt}
\begin{tabular}{|cccc|}
\multicolumn{4}{c}{Batch size 64, 7B params} \\
\hline
Num \vspace{-2 pt} & Time & FLOPS & FLOPS \vspace{-2 pt} \\ 
 Mach. & (secs) &  & /mach. \\ 
       \hline
1 &	224 & 9.28e11 &  9.68e11 \\
2 &	97 & 2.23e12 & 1.11e12 \\
4 &	50 & 4.33e12 &  1.08e12 \\
8 &	28 & 7.74e12 &  9.68e11 \\
       \hline
\end{tabular}
    \end{minipage}%
    \vspace{-5 pt}
    \caption{Performance of LLaMA 7B for first-token inference, using \texttt{Einsummable} on a CPU cluster. Sequence length 512 tokens.}
    \label{fig-7B-batch-sisze}
     \vspace{-10 pt}
\end{figure*}

\begin{figure*}[th!]
    \centering
    \begin{minipage}{.37\textwidth}
        \centering
        \setlength\tabcolsep{3pt}
\begin{tabular}{|cccc|}
\multicolumn{4}{c}{CPU, batch size 1, 65B params} \\
\hline
Num \vspace{-2 pt} & Time & FLOPS & FLOPS \vspace{-2 pt} \\ 
 Mach. & (secs) &  & /mach. \\ 
       \hline
2 &	22.3 & 1.50e12 &  7.51e11 \\
4 &	13.5 & 2.48e12 & 6.20e11 \\
8 &	8.12 & 4.17e12 &  5.16e11 \\
16 & 8.05 & 4.16e12 & 2.60e11 \\
       \hline
\end{tabular}

\end{minipage}%
    \begin{minipage}{.25\textwidth}
    \centering \setlength\tabcolsep{3pt}
\begin{tabular}{|cccc|}
\multicolumn{4}{c}{Batch size 4, 65B params} \\
\hline
Num \vspace{-2 pt} & Time & FLOPS & FLOPS \vspace{-2 pt} \\ 
 Mach. & (secs) &  & /mach. \\ 
       \hline
2 &	73.9 & 1.81e12 &  9.06e11 \\
4 &	33.4 & 4.06e12 & 1.01e12 \\
8 &	24.0 & 5.59e12 & 6.98e11 \\
16 & 15.2 & 8.82e12 &  5.51e11 \\
       \hline
\end{tabular}

    \end{minipage}%
    \begin{minipage}{.37\textwidth}
        \centering   \setlength\tabcolsep{3pt}
\begin{tabular}{|cccc|}
\multicolumn{4}{c}{Batch size 16, 65B params} \\
\hline
Num \vspace{-2 pt} & Time & FLOPS & FLOPS \vspace{-2 pt} \\ 
 Mach. & (secs) &  & /mach. \\ 
       \hline
2 &	509 & 1.05e12 &  5.27e11 \\
4 &	180 & 2.98e12 & 7.45e11 \\
8 &	98.8 & 5.416e12 &  6.77e11 \\
16 & 43.0 & 1.24e13 &  7.79e11 \\
       \hline
\end{tabular}
    \end{minipage}%
      \vspace{-5 pt}
    \caption{Performance of LLaMA 65B for first-token inference, using \texttt{Einsummable} on a CPU cluster. Sequence length 512 tokens. }
        \label{fig-65B-batch-sisze}
         \vspace{-5 pt}
\end{figure*}



\subsection{A Dataflow Approach}

Thus, we use a fine-grained dataflow approach \cite{dennis1980data,karp1966properties}. First, the \textsc{TaskGraph} is ``exploded.''
That is, each EinSum operation is 
expanded into a lineage graph that explicitly shows data flow from tuple to tuple; the various EinSum operations are connected via subgraphs that implement the repartitions between operations.  The vertices in the resulting \textsc{ExecGraph} represent atomic computations over tuples (kernel calls) and edges represent data flow.   These vertices are carefully placed on machines where they are to be executed.  Note that in a CPU cluster, processors will correspond to CPU cores, whereas a ``machine'' is typically the set of processors that have access to the same memory bank, and so they do not need to communicate through a slow network.  The placement is performed so that (1) all machines have a similar amount of work, and (2) so that communication is minimized.  This is considered in detail in the next section of the paper. 


In \texttt{Einsummable}, an \textsc{ExecGraph} is executed asynchronously by a  single-threaded \emph{event loop} whose job is to monitor when the dependencies implicit in the \textsc{ExecGraph} are satisfied. When the inputs to a vertex are found to be available, the event loop will check to see if the resources necessary to execute the vertex are also available (a ``resource'' may be an unoccupied CPU thread, for example, or an open communication channel).  If resources are available, the event loop may choose to execute the vertex.  We use the term ``event loop'' because the loop  asks the necessary resources to execute the vertices in the \textsc{ExecGraph} in response to ``events.'' An event occurs whenever a dependency in the graph has been satisfied, or when a resource that was previously being used becomes available.  
In the case of multi-machine (distributed) execution, there is one event loop per machine, and the event loop also contains vertices that perform communication.  


\subsection{The Importance of Asynchronicity}  

In many proposals for high-performance, distributed/parallel ML \cite{zheng2022alpa,sergeev2018horovod}, there are distinct phases, where an operation such as matrix multiplication is first executed as a number kernel calls, after which an aggregation phase begins.  Aggregation is communication heavy, whereas the pairwise matrix multiplies are computation heavy.  During each phase, resources go unused.  Other systems resort to using protocols such as ring all-reduce \cite{sergeev2018horovod} to reduce the latency of the communication/aggregation phase.

In \texttt{Einsummable}, execution of an \textsc{ExecGraph} is fully asynchronous and aggregations begin any time that the relevant dependencies are satisfied.  In a matrix multiply, for example, \texttt{Einsummable} begins executing the aggregation while pairwise matrix multiply kernel calls are still executing. This allows \texttt{Einsummable} to  effectively overlap communication and computation.

%A related issue is that as a computation is run, the \texttt{Einsummable} event loop will frequently find that at a given moment, many different vertices can be executed. When alternatives are available, we have found that traversing each \textsc{ExecGraphPM} depth-first can have significant benefits in terms of reducing overall execution time, because it means that the system then tends to have very different types of vertices executing at a given instant---ensuring that different types of resources are in use at all times.  A breadth-first traversal, in the other hand, results in an execution that may resemble the ``phases'' executed by other systems. Using a depth-first strategy, the system would first try to finish all of the pairwise matrix multiplies, and only after they all finish, start on the aggregation. 



==> Intro.tex <==

Modern machine learning (ML) systems such as TensorFlow \cite{AbadiBCCDDDGIIK16} and PyTorch \cite{PaszkeGMLBCKLGA19} have high performance.  But they but have significant limitations for large-scale ML. These systems require a programmer to manually decompose ML computations so that they can run on multiple machines or GPUs \cite{tfdist,shazeer2018mesh}. This can be very challenging in the case of modern, large language models \cite{shoeybi2019megatron}.  Moving from one hardware setup to the next in a distributed setting requires writing a lot of code.  Because ML systems cannot decompose computations into smaller parts that can be paged in and out of RAM, out-of-memory problems plague ML programmers \cite{rajbhandari2021zero}.  

TensorFlow and PyTorch are relational systems, operating over \emph{tensors}\footnote{The term \emph{tensor} can mean different things to different scientists and engineers.  For example, to a physicist, it may be a multilinear map (a type of function).  But to an ML engineer, it is typically just a data structure; that is how we use the term here.}, which are relations mapping keys (lists of integers that index into the tensor) to values, typically single or half-precision floats. Yet the aforementioned problems are mostly absent in relational databases. However, few would seriously consider using a relational database engine as an alternative to TensorFlow and PyTorch, as a relational database engine would be too slow.  TensorFlow and PyTorch make use of high-performance, hardware specific kernel functions for operations such as matrix multiplication to achieve performance that no relational database system can match.

Ideally, there would exist a relational system that has the best characteristics of both: all of the automation and scalability of a relational database, with the performance of an ML system. We propose a new type of hybrid relational system called \texttt{Einsum\-mable} that utilizes high-performance kernels like an ML system but offers a fully declarative programming interface, and can automatically decompose a computation, adapting to the available hardware, like a relational database system.

\vspace{3 pt} 
\noindent
\textbf{Dense tensors vs. sparse tensors.} 
Tensors in ML systems are typically \emph{dense}---all possible key values are present in the relation---and database relations  are \emph{sparse}---only a tiny subset of the possible key values are present.  
  Consider the matrix (2-dimensional tensor): $$ \textbf{U} = \begin{bmatrix}
1.4 & 2.2 & 0 & 2.1 \\
2.3 & 2.6 & 1.1 & 2.2\\
1.4 & 1.0 & 1.1 & 1.4 \\
1.1 & 1.4 & 2.5 & 2.3
\end{bmatrix}$$ 
In ML systems, such tensors are stored in arrays, where keys are implicit in the position.  For example, we may store a matrix (a two-dimensional tensor) $\textbf{U}$ in row-major form, meaning that it is stored as an array-of-row-arrays: $\textbf{U} \equiv \langle \langle 1.4, 2.2, 0, 2.1 \rangle$, $\langle 2.3, 2.6, 1.1, 2.2 \rangle, ...\rangle$.  
In contrast, classical relational database management systems operate over relations that have been decomposed into un-ordered sets of ``tuples'', where keys are represented explicitly: $\textbf{U} \equiv \{(\langle 1, 1\rangle, 1.4), \langle 1, 4\rangle, 2.1), \langle 2, 2\rangle, 2.6), ...\}.$ 

This seemingly minor difference has major implications. Because there is no ordering in a relational database, 
locating a tuple in a large relation may be difficult, and require use of an indexing structure, such as a B+Tree.  However, this lack of ordering can be an advantage.  Keys are explicit and order does not matter,  so both tuples and operations are easily distributed over multiple machines or devices.  Efficient parallel/distributed implementations of the classic set of relational algorithms (especially joins and aggregations) rely on sorting or hashing tuples based upon key values, to move them to exactly the location where they can be operated over. 
Such algorithms can scale to very large data sets, even data sets that are larger than the available main memory \cite{kossmann2000state}.  

In contrast, array-based computations have pre-defined memory layouts enabling high-performance special-purpose codes for important operations such as matrix multiplication---or ``kernels'' \cite{vasilache2018tensor,kjolstad2017tensor,chen2018tvm}. There is a high CPU overhead to push each tuple through a relational system \cite{neumann2011efficiently,sompolski2011vectorization,luo2018scalable}. The carefully-designed memory access patterns in an array-based kernel means that a CPU or GPU operates at close to its optimal floating-point operation per second rate, with little overhead.   

\vspace{3 pt} 
\noindent
\textbf{The hybrid tensor-relational approach.}
It is possible to define a \emph{tensor-relational} implementation \cite{yuan2021tensor} that has the benefits of both the array-based approach (enabling the use of high-performance kernels), and the purely relational (easy distribution). Intuitively, the idea is that rather than relying on sets of scalars---as in the relational implementation---we rely on sets of explicitly-keyed chunks:  \begin{align} \textbf{U} \equiv &\Bigg\{ \left( \langle 1, 1 \rangle, \begin{bmatrix} 1.4 & 2.2 \\ 2.3 & 2.6 \end{bmatrix}  \right),
        \left( \langle 1, 2 \rangle, \begin{bmatrix} 0 & 2.1 \\ 1.1 & 2.2 \end{bmatrix}  \right),\nonumber \\ 
        &\left( \langle 2, 1 \rangle, \begin{bmatrix} 1.4 & 1.0 \\ 1.1 & 1.4 \end{bmatrix}  \right),
        \left( \langle 2, 2 \rangle, \begin{bmatrix} 1.1 & 1.4 \\ 2.5 & 2.3 \end{bmatrix}  \right) \nonumber
\Bigg\}.\end{align}
Large tensors can be decomposed into sets of chunks that are easily distributed to multiple sites, or multiple devices, using classical distributed algorithms \cite{kossmann2000state}. However, the fact that sub-tensors are stored in tuples means that high-performance kernels can be used. If we store two matrices \textbf{B} and \textbf{C} as tensor relations using the schema \texttt{(rowID, colID, value)} where \texttt{value} is a matrix, then assuming \texttt{SUM} performs efficient matrix addition and \texttt{matrix\_multiply} calls an appropriate kernel, then \textbf{B} and \textbf{C} can be multiplied using SQL:

\begin{SQL}
SELECT SUM (matrix_multiply (B.val, C.val))) 
FROM B, C WHERE B.colID = C.rowID 
GROUP BY B.rowID, C.colID
\end{SQL}

\noindent
\textbf{\texttt{Einsummable}: The hybrid tensor-relational system.}  In this paper, we describe \texttt{Einsummable}, which is a system for high-perform\-ance distributed ML. \texttt{Einsummable} automatically decomposes ML computations and executes them as tensor-relational computations.  

To date, our primary use case for \texttt{Einsummable} is low-latency inference for large language models (LLMs).  Compared to training, LLM inference is particularly challenging to parallelize \cite{pope2023efficiently}. Latency is a key consideration---some consumer is waiting for the result of LLM inference---and inference is not easily parallized.  In contrast, as each training batch typically backpropagates over a large number of independent data points,  methods such as pipeline parallelism can be used to achieve high training throughput.

While all of the ideas in this paper are applicable to both CPU and GPU computation, our \texttt{Einsummable} prototype focuses on CPUs, which have the advantage of scaling to very large inference tasks far more economically than GPUs. For example, first-token inference with a 100,000 token prompt for the 65-billion parameter LLaMA model \cite{touvron2023llama} requires an attention computation whose results alone take up at least 1.3TB of RAM.  To run such a computation in GPU RAM would likely take at least 20 A100 GPUs, each of which with 80GB of RAM.  At 2023 prices, these 20 GPUs (without any other hardware) would cost around half a million US dollars.  In contrast, one could purchase 16 reasonably performant Intel Xeon CPUs and 3TB of DDR4 RAM for significantly less than \$50,000.


\vspace{3 pt} 
\noindent
\textbf{Challenges in tensor-relational system construction.}
While a tensor-relat\-ion\-al implementation for large-scale ML can potentially realize the advantages of both the array-based and relational implementations, there are a series of challenging problems to solve:

\vspace{3 pt}
\noindent
\textit{A tensor-relational system must be able to ``understand'' the underlying ML computation in order to optimize it.} TensorFlow and PyTorch programmers call black-box operations (such as \texttt{torch.matmul}), hence the system is unable to reason about the correct way to implement the computation. Instead, a declarative language is needed. One could ask an ML engineer to program a tensor-relational system using SQL, but that seems unreasonable. \texttt{Einsummable} asks programmers to use a variant of the Einstein summation notation \cite{blacher2023efficient,laue2020simple,einstein1938gravitational} to declaratively specify their ML computations.

\vspace{3 pt}
\noindent
\textit{We cannot expect a programmer to choose how to decompose a pure, array-based computation.}  Yet the decomposition of tensors into relations, can have profound performance considerations.  How can a tensor-relational system automatically optimize the schema design process?  \texttt{Einsum\-mable} minimizes an upper bound on the amount of communication required to implement the  computation.

\vspace{3 pt}
\noindent
\textit{Traditional relational algorithms---sort merge joins, hash-based aggregation, etc.---are not ideal for implementing tensor-relational computations}. They assume large numbers of small tuples, not a small number of sub-tensors.  What should a tensor-relational engine look like?  \texttt{Einsummable} uses a data-flow style engine \cite{karp1966properties}, along with an algorithm that carefully places operations in a distributed system to minimize communication and ensure load balancing.

\vspace{3 pt} 
\noindent
\textbf{Our contributions.}  We design, prototype and  evaluate  \texttt{Einsum\-mable}.  Over a comprehensive set of experiments involving serving the LLaMA \cite{touvron2023llama} large language model \cite{zhao2023survey}  using \texttt{Einsummable}-based CPU cluster, we show that \texttt{Einsummable} is able to effectively parallelize LLM inference, without human involvement, past the declarative specification of the  LLaMA model.

==> Old_Abstract.tex <==

Modern machine learning (ML) systems such as TensorFlow and
PyTorch are relational systems. ML systems operate over tensors,
which are relations mapping positions to values.  ML systems are very high-performance for modern deep learning computations, but unlike relational databases, ML systems are quite poor at dealing with limited memory, and automatic optimization and parallelization. In this paper, we describe \texttt{Einsummable}, which is a new tensor-relational system that has the benefits of classical relational databases (easy scalability, automatic parallelism) as well as the benefits of ML systems (high performance).  We implement \texttt{Einsummable} for clusters of CPU machines, and extensively benchmark its ability to serve large language models.  We find that it can automatically scale to very large inference tasks.

==> Overview.tex <==

Compared to other systems for automatically decomposing ML computations for the purpose of facilitating parallelism and/or memory management \cite{zheng2022alpa,rajbhandari2021zero,xu2021gspmd}, \texttt{Einsummable} is unique in that it starts with a fully declarative programming abstraction.  This programming abstraction is a graph of mathematical expressions, specified using an extended Einstein summation notation.  We call this graph an \textsc{EinGraph} (formally defined in Section 3 of the paper). The  \textsc{EinGraph} is pushed through a series of compilation steps to obtain a dataflow graph that can be executed on \texttt{Einsummable}'s asynchronous, event-based back-end.  Any mathematical computation expressed as a graph in our extended Einstein summation notation can be processed using the \texttt{Einsummable} system.

The most obvious implementation of an \textsc{EinGraph} would be as a series of joins and aggregations over fully normalized tuples.  However, this would not be efficient, so \texttt{Einsummable} takes a tensor-relational approach. \texttt{Einsummable} annotates the \textsc{EinGraph} with specifications for the optimal decomposition of each vertex.  This creates a \textsc{TaskGraph} (see Section 4) which is equivalent to the original \textsc{EinGraph}, but specifies a series of joins and aggregations over tensor relations, whose tuples store sub-tensors.  This annotation is done so as to minimize an upper bound on communication in a generic, parallel implementation (see Section 5). 
Executing the \textsc{EinGraph} on a classical relational engine would be sub-optimal.  Thus, we instead compile the \textsc{EinGraph} into a fine-grained dataflow graph, which is executed asynchronously, allowing the overlapping of communication and computation (Section 6) This is done to ensure load balancing and to minimize communication (Section 7).
